Public Transport Planning: When Transit Network Connectivity Meets Commuting Demand

In this paper, we make a first attempt to incorporate both commuting demand and transit network connectivity in bus route planning (CT-Bus), and formulate it as a constrained optimization problem: planning a new bus route with k edges over an existing transit network without building new bus stops to maximize a linear aggregation of commuting demand and connectivity of the transit network. We prove the NP-hardness of CT-Bus and propose an expansion-based greedy algorithm that iteratively scans potential candidate paths in the network. To boost the efficiency of computing the connectivity of new networks with candidate paths, we convert it to a matrix trace estimation problem and employ a Lanczos method to estimate the natural connectivity of the transit network with a guaranteed error bound. Furthermore, we derive upper bounds on the objective values and use them to greedily select candidates for expansion. Our experiments conducted on real-world transit networks in New York City and Chicago verify the efficiency, effectiveness, and scalability of our algorithms.

==> Optimization.tex <==
%\section{Optimization}

%\subsection{Approximate algorithm}
%Approximate ratio of new algorithm. 
%We aim to satisfy fair representation while approximately preserving the objective.
%According to the state-of-the-art, there is still no proved ratio for k-TSP problem.

\section{Budget-based FairBus}
\label{sec:budget}
A single route planning aims to cover the newly founded edges in a single bus route, which works well when those new edges show a similar trend.
However, in the experiments, we found some edges are far from each other, and it also takes a long distance to connect them and produce bigger objective value and also detours.
Planning multiple routes can effectively resolve this problem; we define it as budget-based \fairbus.

\subsection{Definition}
%Budget-based route planning: designing k new routes rather than a single route.
We can revise the definition of \fairbus to find $k$ routes, and the fairness constraint does not change, i.e., the same number of edges will be added. The objective functions will change as below:

\begin{equation}
\label{equ:budget}
O_1=\argmin_{\mu_1,\cdots, \mu_k\in G }{{\sum_{j=1}^{k}\sum_{T_i\in S_j}{\var{Dist}(T_i,\mu_j)}}}%, \frac{\epsilon(G_r^{'})-\epsilon(G_r)}{\epsilon(G_r)}\ge\Delta%\epsilon(\mu)\in [\epsilon_{min}, \epsilon_{max}]
\end{equation}
where $G_r^{'} =\{V, E\cup \{\mu_1, \cdots, \mu_k\}\}$.

The solutions can be very similar, and the detection framework can be used in the same way.
%We can conduct k-paths clustering to generate k weighted graph.
To choose a parameter $k$, we aim to divide the founded edges into groups of the path that has the highest combinable potential, based on direction, and districts in the city, e.g., New York has five districts and each district has its bus systems. Given $k$ sets of edges, conducting \fairbus query individually is a solution.

\subsection{Dividing New Edges into $m$ sets}
To group the edges, we consider the direction factors and avoid detours.
Grouping can also reduce the number of candidates from $|C|!$ to $\sum_{i=1}^k |C_i|!$, where $C_i$ is the sub-group and $\sum_{i=1}^k |C_i|=|C|$.

%Our solution is to build matrix, and infer the sub-groups.

Proving that dividing into groups will decrease the objective value further is crucial, rather than using a case study.
A baseline is to try every permutation, then call the method in last section. However, complexity is high.
How to prune candidates and guarantee that it will not be results.
We can estimate the bound, e.g., far edges being connected will make the route very long, so it  will exceed the bound, so we should not connect them.
We can estimate the length bound to group edge segments into limited number of edges, then bound all the edges within a distance, and also minimize the travel length.

\subsection{Revised \dcep}
The main difference with Algorithm~\ref{alg:fairbus} is that we need to maintain $k$ queues and global objective value.
To avoid overlaps between the routes, we take a sequential scanning method.

\iffalse
\subsection{Round-Trip Bus Routes}
We can loss the expansion constraint, by converting the road network and transit network into undirected graphs, where the weight will be the sum of two directions.
During the traversal, we add constraint checking, e.g., length of route, building new stops, minimum number of routes.
Constraint-based planning by considering building new stops.
Through analysis, we found that the founded route's two adjacent stops are too far, and may need to build new stops.
We set a threshold distance, 
When there is budget to build several new stops and update $G_R$, how to select proper locations and further form a route that can further maximize the objective functions.
We introduce a new parameter $N_s$, it is the number of new stops
The bus route length cannot be too long due to the normalization in the distance measure.
\fi



==> append.tex <==

\begin{figure*}[h]
	\centering
	\includegraphics[width=16cm]{graph/ahead.pdf}\vspace{0.5em}\\
	%	\includegraphics[width=0.33\linewidth]{graph/30_3_3_5000.pdf}
	%	\includegraphics[width=0.33\linewidth]{graph/30_5_3_5000.pdf}
	%	\includegraphics[width=0.33\linewidth]{graph/30_7_3_5000.pdf}\\ \vspace{1em}
	%	\includegraphics[width=5.2cm]{graph/30_5_3_5000.pdf}
	\includegraphics[width=0.32\linewidth]{graph/50_5_3_5000.pdf}
	\includegraphics[width=0.32\linewidth]{graph/80_5_3_5000.pdf}
	%	\includegraphics[width=5.2cm]{graph/30_5_3_5000.pdf}
	\includegraphics[width=0.32\linewidth]{graph/30_5_5_5000.pdf}\\\vspace{0.5em}
	\includegraphics[width=0.32\linewidth]{graph/30_5_1_5000.pdf}
	\includegraphics[width=0.32\linewidth]{graph/30_5_3_3000.pdf}
	%	\includegraphics[width=5.2cm]{graph/30_5_3_5000.pdf}
	\includegraphics[width=0.32\linewidth]{graph/30_5_3_7000.pdf}\\
	\vspace{-1em}
	\caption{Supplementary parameter-sensitivities experiments on $k$, $\var{Tn}$ (number of turns), and $\var{sn}$ (seeding number).}
	\vspace{-1em}
	\label{fig:efficiency1}
\end{figure*}

\section{Proof of Lemmas}
\subsection{Proof of Lemma~\ref{lem:np}}

\begin{proof}
	When $G_r$ is a fully connected graph (complete graph), i.e., the connectivity will not change, then we only optimize over $O_d$ for \fairbus, which can be reduced to the \textit{minimum k-TSP problem} which has been proved to be NP-hard: \textit{Choosing a path to maximize the sum score problem with a limited number ($k$) of vertexes is known as $k$ minimum travel salesman problem (k-TSP) \cite{Arora,Garg2005}}.
	
	Further, optimizing one objective can be converted to a  $k$-TSP problem, which is already NP-hard. Our \fairbus that optimizes two objectives simultaneously is at least as hard as optimizing one objective, thus is also NP-hard.
\end{proof}


\subsection{Proof of Lemma~\ref{lem:general_edge_additions}}

\begin{proof}
	Let $\bm{A}$ be the adjacency matrix of our original transit network $G_r$ and let $\bm{A}'$ be the adjacency matrix of the updated network $G_r'$, which is obtained by adding $k$ edges.
	Let $\bm{K} = \bm{A}'-\bm{A}$. Let $\lambda_1 \geq \ldots \geq \lambda_n$, $\lambda_1' \geq \ldots \geq \lambda_n'$, and $\sigma_1 \geq \ldots \geq \sigma_n$ be the eigenvalues of $\bm{A}$, $\bm{A}'$, and $\bm{K}$, respectively.
	
	Let $\tr(\cdot)$ denote the matrix trace, we have $\lambda(G_r') = \ln\left(\frac{1}{n}\tr(e^{\bm{A}'})\right)$. Then it suffices to upper bound $\tr(e^{\bm{A}'})$. To do so, we apply the Golden–Thompson inequality: $\tr(e^{\bm{A}'}) = \tr(e^{\bm{A}+\bm{K}}) \leq \tr(e^{\bm{A}}e^{\bm{K}})$. Next, we apply a trace inequality of Lassere \cite{lasserre1995trace} to bound
	$\tr(e^{\bm{A}}e^{\bm{K}}) \leq \sum_{i=1}^ne^{\lambda_i}e^{\sigma_i}$. Since $\bm{K}$ is a graph adjacency matrix with at most $2k$ nodes, it has a rank of at most $2k$, so we have $\sum_{i=1}^n e^{\lambda_i} e^{\sigma_i} \leq \sum_{i=2k+1}^n e^{\lambda_i} + e^{\lambda_1}\sum_{i=1}^{2k} e^{\sigma_i}$. Since this expression is maximized exactly when $\bm{K}$ is chosen to maximize the Estrada index $\sum_{i=1}^{2k} e^{\sigma_i}$, we can apply the upper bound of \citet{DeLaPena2007} to obtain $\sum_{i=1}^{2k} e^{\sigma_i} \leq 2k - 1 +e^{\sqrt{2k}}$.
	
	Our final result is that $\tr(e^{\bm{A}'}) \leq \tr(e^{\bm{A}}) - \sum_{i=1}^{2k} e^{\lambda_i} + e^{\lambda_1}[2k - 1 +e^{\sqrt{2k}]}$, which gives the bound of the lemma after renormalizing and taking a log.
\end{proof}


\subsection{Proof of Lemma~\ref{lem:path_edge_additions}}

\begin{proof}
	For $i = 1,\ldots, n$, let $\Delta_i = \lambda_i' - \lambda_i$. We have that:
	\begin{align}
	\label{eq:to_max}
	e^{\lambda(G_r')} = e^{\lambda(G_r)} + \frac{1}{n}\sum_{i=1}^{n} (e^{\Delta_i} - 1)e^{\lambda_i}. 
	\end{align}
	We are going to choose $\Delta_1^*, \ldots, \Delta_n^*$ to maximize this expression given the constraints of implied by Equation \ref{eq:ky_fan}:
	\begin{align*}
	&\text{For all $q = 1,\ldots, n$,} & \sum_{i=1}^q \Delta_i &\leq \sum_{i=1}^q \sigma_i.
	\end{align*}
	It is clear that any solution which maximizes Equation~\ref{eq:to_max} under these constraints must set $\Delta_q^* = \sum_{i=1}^q \sigma_i - \sum_{i=1}^{q-1} \sigma_i = \sigma_q$. 
	
	The non-zero eigenvalues of $\bm{K} = \bm{A}'-\bm{A}$ are simply the well-known eigenvalues of an unweighted simple path graph, which are equal to $2\cos\left(\frac{i\pi}{k+2}\right)$ for $i = 1,\ldots,k+1$. The remaining $n-k-1$ eigenvalues of $\bm{K}$ are equal to $0$.
	Noting that only the first $m = \lfloor\frac{k+1}{2}\rfloor$ path graph eigenvalues are positive, we immediately have that $\Delta_1^*, \ldots \Delta_{m}^* = 2\cos\left(\frac{1\pi}{k+2}\right), \ldots, 2\cos\left(\frac{m\pi}{k+2}\right)$, $ \Delta_{m+1}^*, \ldots,\Delta_{n-k+m}^* = 0$, and $\Delta_{n-k+m+1}^*,\ldots, \Delta_{n}^* =\allowbreak 2\cos\left(\frac{(m+1)\pi}{k+2}\right), \ldots, 2\cos\left(\frac{(k+1)\pi}{k+2}\right)$.
	
	The lemma follows by noting that $(e^\Delta_i - 1) \leq 1$ for all $\Delta_i \leq 0$.
\end{proof}



\begin{comment}
	\centering
	\caption{{Summary of notations.}}
%	\vspace{-1em}
	\label{tab:notation}
	\scalebox{0.94}{\begin{tabular}{cc}
			\toprule
			\textbf{Symbols}    & \textbf{Description}                                   \\ \midrule
			$T_i$, $D$       & A trajectory, and the dataset                          \\ \midrule
			%     $|T_i|$        & The travel length of trajectory $T_i$                \\ \midrule
			$G$, $E$, $V$   & The road network, edges, vertices             \\ \midrule
			$G_r$, $E_r$, $V_r$   & The transit network, edges, vertices             \\ \midrule
			%	      $O$   & The equity objective function                       \\ \midrule
			%		 $a^{'}(i)$, $a(i)$   & $T_i$'s previously and newly assigned cluster ids        \\ \midrule
			$w$, $sn$, $Tn$, $\tau$ & \makecell{The weight, seeding number, \\ threshold on number of turns, \\stop interval distance} \\ \midrule
			$\mu$, $cp$ & The optimal bus route and candidate path   \\ \midrule
			$\bm{A}$, $n$, $\lambda_i$ & Adjacent matrices, dimension, $i$-th eigenvalue \\ \midrule
			$L_d$, $L_\lambda, L_e$ & \makecell{Descending sorted list of edges by demand, \\connectivity and equity objective increment}\\ \midrule
			\makecell{$\ub(cp)$, \\ $\ub_d(cp)$, $\ub_\lambda(cp)$} & \makecell{The upper bound of equity objective value, \\ demand, connectivity of candidate path $cp$ }\\ \midrule
			$tn(cp)$, $cur$ & \makecell{Number of turns, \\and bound cursor of candidate path $cp$ }
			\\
			\bottomrule
	\end{tabular}}
\end{comment}


\section{Implementation}
We use Python 3 to clean data and search the shortest paths between two stops, and MATLAB to compute the connectivity, which is much faster in term of large matrix computation. %\bao{how about the PL for the rest part?}
%For existing edges, we map the bus route to the road network and sum up the demand for each edge.
NetworkX\footnote{\url{https://networkx.github.io}} is used to store the graph and shortest path, and
Mapv\footnote{\url{https://github.com/huiyan-fe/mapv}} is used to visualize the networks and the returned results in maps.
All experiments are conducted on a laptop with 2.6 GHz 6-Core Intel Core i7 and 32 GB 2400 MHz DDR4 running MacOS Catalina.
Our cleaned datasets, MATLAB code, and visualization tools are all available on GitHub for reproducibility.\footnote{\url{https://github.com/tgbnhy/EquaBus-code}}
% \cite{Hagberg2008}

\begin{algorithm}
	\caption{Increment demand bound \& turn update}
	\KwIn{$e$, $\ub_d(cp)$, $tn(cp)$, $cur$}
	%	\KwOut{$UB(ps)$, $Tn(ps)$, $cur$}
	\label{alg:bound}
	\If{$L_d(cur)>L_d[e]$}
	{
		$cur \leftarrow cur-1$\;
		$\ub_d(cp) \leftarrow \ub_d(cp)-({L_d(cur)-L_d[e]})$\;
	}
	$angle\leftarrow \textsc{ComputeAngle}(e, cp.end)$\;
	\If{$angle>\frac{\pi}{4}$}
	{
		$tn(cp)\leftarrow tn(cp)+1$\;
	}{
		\If{$angle>\frac{\pi}{2}$}{$tn(cp)\leftarrow \var{Tn}$\;}
	}
	\Return $\big(\ub_d(cp), tn(cp), cur\big)$\; 
\end{algorithm}
%edge is an important factor.

\section{Pre-processing}
Table~\ref{tab:precom} shows the number of new edges of our two datasets, and pre-processing time on them.
Pre-processing on the candidate new edges includes time spent on the shortest path search of selective new edges, and their connectivity increment based on the Lanczos method.
Each new edge conducted the shortest path between its two ends, then we put the edge demand by summing up edges in the road network; 
Even though the pre-computation costs much time, it is called only once for each dataset and will benefit all the algorithms with various parameter settings.

\begin{table}[t]
	\caption{Running time of pre-computation on new edges.}
	\vspace{-1em}
	\label{tab:precom}
	\scalebox{0.95}{\begin{tabular}{cccc}
		\toprule
		\textbf{Method} &  \textbf{\makecell{\#New edges}} & \textbf{Connectivity}  & \textbf{\makecell{Shortest path \\search}} \\
		\midrule
		Chicago & 95,304 & 1857s &15,322s \\
		NYC & 160,790& 7332s  & 33,241s  \\
		\bottomrule
	\end{tabular}}
\end{table}


\begin{figure}
	\vspace{-0.5em}
	\centering
	\subfigure[Chicago]{\includegraphics[height=2.5cm]{graph/topkchi.PNG}}~~~~~\hspace{1em}
	\subfigure[NYC]{\includegraphics[height=2.5cm]{graph/topknyc.PNG}}
	\vspace{-1.5em}
	\caption{Top-$10$ edges returned by a greedy algorithm {Chan2014}.}
%	\vspace{-1em}
	\label{fig:baseline-topk}
\end{figure}


\begin{figure}
	\centering
	%	\vspace{-1em}
	\includegraphics[height=3cm]{graph/chi-connectivity.pdf}
	\includegraphics[height=3cm]{graph/nyc-connectivity.pdf}
	\vspace{-1em}
	\caption{Evaluation of natural connectivity on real datasets.}
	\vspace{-1em}
	\label{fig:connectivity}
\end{figure}


\section{More Parameter Sensitivity Test}
In Figure~\ref{fig:efficiency1}, we add more experiments on parameter sensitivities,
where we can observe the equity drop with the increasing of $k$, this is because our normalization values $d_{max}$ and $\lambda_{max}$ also rise as they are related to $k$ in Equation~\ref{equ:newb}, but with an increase rate bigger than $O_d$ and $O_\lambda$.
Other parameters $w$, $\var{Tn}$, and $\var{sn}$ do not have much affect on the convergence.

%Experiments on radius $\tau$ in two datasets,  
%\section{More case studies}

\section{More Discussions}

\myparagraph{Complexity Comparison of ETA}
Firstly, our method is independent of the number of trajectories $|D|$, as all the trajectories are mapped to the road network and each road-network edge gets a demand weight.
The pre-processing on mapping and building transit network edge weight is related to the number of new edges, as each edge will call one time shortest path search, and connectivity increment estimation using the Lanczos method.

For the \textbf{ETA} algorithm in Section 4, the complexity of each iteration is related to the connectivity and bound estimation, the connectivity estimation needs to be conducted for every neighbor edge. Bound estimation needs to be conducted once. 
This can be ignored with our pre-computation proposed in this section.
%\sheng{Complexity equation here based on chris's.}

\myparagraph{Effect of Increasing $\tau$}
According to the above analysis, the complexity of \fairbus is highly related to the number of candidate edges.
A direct parameter to this is the neighbor stop interval distance $\tau$ in Definition~\ref{def:fairbus}; if we increase $\tau$, there will be more candidate edges.
In this paper, we set $\tau$ as a fixed constant $0.5$km, which is already a big value in current statistics in NYC.
However, the number of edges will not sharply increase according to our initial numerical analysis, the running time of pre-computation and ETA will increase linearly and slightly when increasing $\tau$ in a proper range.
%We skip the results here due to space limit.

\myparagraph{Planning Multiple Routes}
\fairbus is also flexible to plan multiple routes by calling it incrementally.
After planning a new route, we update the graph and its adjacent matrix with the new edges.
Then, we put all the covered edges' demand value as zero, as our last planned new bus routes have covered them.
In the end, we conduct the new route searching using our algorithm.

\myparagraph{Future Work}
In future, we will investigate how to update the connectivity efficiently in the pre-computation based on perturbation theory,  and use our derived upper bounds to solve existing and new network connectivity optimization problems \cite{Chan2014,Chen2018d}.
Further, we will set the optimal timetable for the new route to reducing the waiting time to transfer to other crossed routes, by considering the temporal dimension of trajectory data.
For some small-scale cities which do not have sophisticated transit systems like NYC, 
the optimal site selection for deploying new bus stops based on trajectories and connectivity will be another interesting problem.


%More evaluations.
